DLAS: An Exploration and Assessment of the Deep Learning Acceleration Stack

Deep Neural Networks (DNNs) are extremely computationally demanding, which presents a large barrier to their deployment on resource-constrained devices. Since such devices are where many emerging deep learning applications lie (e.g., drones, vision-based medical technology), significant bodies of work from both the machine learning and systems communities have attempted to provide optimizations to accelerate DNNs. To help unify these two perspectives, in this paper we combine machine learning and systems techniques within the Deep Learning Acceleration Stack (DLAS), and demonstrate how these layers can be tightly dependent on each other with an across-stack perturbation study. We evaluate the impact on accuracy and inference time when varying different parameters of DLAS across two datasets, seven popular DNN architectures, four DNN compression techniques, three algorithmic primitives with sparse and dense variants, untuned and auto-scheduled code generation, and four hardware platforms. Our evaluation highlights how perturbations across DLAS parameters can cause significant variation and across-stack interactions. The highest level observation from our evaluation is that the model size, accuracy, and inference time are not guaranteed to be correlated. Overall we make 13 key observations, including that speedups provided by compression techniques are very hardware dependent, and that compiler auto-tuning can significantly alter what the best algorithm to use for a given configuration is. With DLAS, we aim to provide a reference framework to aid machine learning and systems practitioners in reasoning about the context in which their respective DNN acceleration solutions exist in. With our evaluation strongly motivating the need for co-design, we believe that DLAS can be a valuable concept for exploring the next generation of co-designed accelerated deep learning solutions.

==> XX-background_old.tex <==
\section{Background}
\label{sec:background}



\begin{figure*}[!ht]
\begin{center}

  \begin{subfigure}{0.21\textwidth}
  	\includegraphics[width=\linewidth]{graphs/fig_dense.eps}
    \caption{Dense Convolutions}
\label{fig_dense}
  \end{subfigure}
    \hspace*{\fill}   %
  \begin{subfigure}{0.21\textwidth}
  \includegraphics[width=\linewidth]{graphs/fig_sparse.eps}
    \caption{Weights Pruning}
  \label{fig_sparse}
  \end{subfigure}
  \hspace*{\fill}   %
  \begin{subfigure}{0.21\textwidth}
     \includegraphics[width=\linewidth]{graphs/fig_fisher.eps}
    \caption{Channel Pruning}
  \label{fig_fisher}
  \end{subfigure}
    \hspace*{\fill}   %
  \begin{subfigure}{0.21\textwidth}
  \includegraphics[width=\linewidth]{graphs/fig_quantiz.eps}
    \caption{Weights Quantisation}
      \label{fig_quantization}
  \end{subfigure}
\caption{A visual representation of different compression techniques: (a) shows a slice of a standard neural network. Each rectangle represents the output generated by convolving filters with learnt weights (parameters) over each input channel; (b) shows the same network slice with weight pruning applied. A subset of weights in the filters are forced to zero (visually represented with white holes) producing sparse matrices; (c) shows the network slice with channel pruning applied onto the middle layer, where the connections remain dense but there are fewer channels; (d) shows the quantisation process for weights, constraining all value from the original distribution to just three possible values (ternary quantisation).} 
\label{fig:systems}
\end{center}
\end{figure*}


A range of compression techniques have been proposed in the Machine Learning community. In this section we present the techniques most relevant to this paper and their variants.

\subsection{Weight pruning} %

Weight pruning is a popular technique for reducing the parameter count in neural networks, and has been shown to improve generalisation~\cite{scardapane2017group}. Weight pruning techniques introduce sparsity in the network and generally fall into two categories: (i) unstructured removal of weights deemed unnecessary; and (ii) structured regularisation --- pushing the network weights towards a regular sparse format. The step from Figure \ref{fig_dense} to \ref{fig_sparse} shows an example of a network with individually pruned weights. %

The removal of redundant weights was first proposed in~\cite{NIPS1988_156}, which uses different biases to penalise the error function used to train the network. A more computationally demanding approach was suggested in~\cite{lecun1990optimal} which involved computing second derivatives to find and remove weights with the smallest effect on the error function.  

A less computationally demanding method is proposed in~\cite{han2015learning}, where the network is trained in its original dense format, and then all weights below a certain threshold are removed. This is applied layer-by-layer, where the threshold is determined by the standard deviation of the layer. The authors show that after pruning, the network should be retrained with its new weights in order to maintain accuracy, and that by iteratively repeating this process they can prune up to 90\% of the weights without affecting accuracy. In~\cite{han2015deep}, this is developed using a three stage method for storing the network involving pruning, quantisation, and Huffman coding.

Other works \cite{liu2015sparse,denil2013predicting} have utilised low-rank approximations that yield significantly reduced sparse networks. The major benefit of this approach is that the network can be kept in a highly optimisable form. In~\cite{liu2015sparse} the authors present a sparse convolution algorithm that can be used along with compression methods to outperform the original dense network. Similarly, \cite{scardapane2017group,wen2016learning} use sparse group Lasso to penalise small weights and push the network towards a structured sparse format. 







\subsection{Channel pruning} %

A natural extension of weight pruning is to not only remove individual weights in a network, but entire channels from the convolutional layers and nodes from the fully connected layers, as shown in Figure \ref{fig_fisher}. One approach to this is to apply Lasso regression to the problem of channel selection~\cite{he2017channel}. This view of channel pruning was questioned by~\cite{ye2018rethinking}, who applied Lasso instead to the batch-norm~\cite{ioffe2015batch} layers of the network and then removed any channels with low batch-norm weights, resulting in greater accuracy. 

Another approach altogether is to approximate the effect of removing certain channels on the error using a \emph{Taylor series} expansion~\cite{molchanov2016pruning,theis2018faster}. Surprisingly, it has been shown that random pruning~\cite{mittal2018recovering} is also an effective strategy for removing filters; many common networks are able to retrain to their original accuracy after iterative stages of randomly removing progressively more filters.


\subsection{Quantisation} %

Quantisation methods attract a lot of attention in the machine learning community due to their immediate impact on memory requirements. In~\cite{zhou_2017_incremental} the number of bits used to represent each weight is reduced --- which we call \emph{data type quantization}. Others have instead restricted each weight to one of several fixed values. HashedNet~\cite{chen_2015_hashing} restricts weights to a smaller set of possible values by using a hash function to map weights to hash buckets, in which they share the same floating point value. The extreme case is achieved by BinaryNet~\cite{courbariaux_2015_binaryconnect} transforming all weights to a one bit representation, with minimal accuracy degradation.  \emph{Log quantization} \cite{miyashita2016,lee2017a} constrains weights to powers of two.  When coupled with complementary optimizations in the \emph{Systems Techniques} layer, multiplication operations can be replaced with bit-shifts - which in many hardware architectures translates to reduced energy consumption and inference time.

These quantisation methods have been proposed and evaluated predominantly on well-known CNNs starting from a floating-point weight representation. The networks are typically pre-trained and then quantisation is applied gradually while fine-tuning (i.e.\ re-training) to maintain a high inference accuracy. This fine-tuning process is essential to compensate for the loss of information in quantising weights. 

Several works observe an increase in network performance after this process, explainable by quantisation acting as a regularisation method in the fine-tuning phase, nudging the quantised model in the right direction in a reshaped convex space. One such promising approach that combines elements from previous quantisation methods is presented in~\cite{zhu_2017_trained}. This ternary quantisation method transforms the weights in convolution filters to just three possible values, the zero value and two other values (one positive and one negative) determined independently for each layer. Figure \ref{fig_quantization} shows an example. %



==> XX-discussion_old.tex <==

\section{Discussion and Related Work}
\label{sec:discussion}

In Section~\ref{sec:evaluation} we observed a large number of variations across our experiments, with a number of non-trivial dynamics emerging.
In this section, we will go through each layer of the stack, and discuss some notable observations from our results, highlighting any potential across-stack interactions, as well promising avenues of research not evaluated in our work.
Our observations are not intended to be definitive, and large changes in our results could be expected by bringing in some other aspect of the stack.
However, this highlights the core thesis of this work: across-stack interactions of machine learning and systems optimizations can be non-trivial, and bringing in additional features may significantly accelerate, or impede the technique.
We refer the reader to other characterization works and surveys which highlight cutting edge techniques from across the stack~\cite{szeEfficientProcessingDeep2020,blalockWhatStateNeural2020,hadidiCharacterizingDeploymentDeep2019,hookerHardwareLottery2021,liDeepLearningCompiler2021,wangConvergenceEdgeComputing2020}.



\subsection{Datasets \& Problem Spaces}

Between datasets, in terms of accuracy, models showed similar trends, with the accuracy losses due to compression being higher for ImageNet models.
The computational requirements of models for each dataset varied, i.e., CIFAR-10 models have fewer MACs than ImageNet (Tables~\ref{tab:acc_cifar10} and~\ref{tab:acc_imagenet}), which we would expect have effects on the behavior elsewhere in the stack.
For instance, when tuned, pruned CIFAR-10 models on the CPU were faster relative to tuned dense \texttt{float32} models, but we did not observe this with ImageNet.
Possible explanations include overheads in our sparse algorithm and data format choices, which could be exacerbated by ImageNet models higher memory and MAC requirements, and the fact that CIFAR-10 models and ImageNet models were given the same number of tuning trials despite the latter being larger.






\subsection{Models \& Neural Architectures}
\label{subsub:discuss:models}

We found that the number of parameters and MACs in a model (Tables~\ref{tab:acc_cifar10} and \ref{tab:acc_imagenet}) did not directly correlate with top-1 accuracy.
For example, EfficientNetB0 has a higher accuracy than both DenseNet161 and ResNet50, despite having at most 21\% of the parameters.
This can be understood as EfficientNetB0 being a more recent model which exploits novel architectural and training techniques to achieve better parameter efficiency.
However other works have shown that if we keep the model architecture the same, more parameters generally means higher accuracy~\cite{crowleyMoonshineDistillingCheap2018,gibsonOptimizingGroupedConvolutions2020,tanEfficientNetRethinkingModel2019}.
Across our experiments, a trend we observed that models with fewer parameters were more vulnerable to accuracy loss when applying compression techniques.

Another observation for EfficientNetB0, is that it had the highest accuracy drops for \texttt{int8} quantization out of any model.
We believe that aspects of EfficientNetB0's architecture are not amenable to post-training quantization.
These issues were highlighted and corrected by EfficientNet-Lite~\cite{liuHigherAccuracyVision2020}, which removes the squeeze-and-excitation networks, and replaces the swish activation functions with ReLU6 activations~\cite{howardMobileNetsEfficientConvolutional2017}, to better support quantization.
The cross-stack interaction here is the choice of model architecture negatively interacting with a compression technique.
Instead of trying to change the quantization approach, the authors opted to change the architecture.


These are also a wide range of other DNN architectures available beyond CNNs.
For example, recurrent neural networks, LSTMs, and Transformers.
Each have their own advantages and disadvantages for different datasets and hardware architectures.
Increasingly, approaches such as Neural Architecture Search (NAS) look to automate the process of finding a network architecture.
EfficientNets~\cite{tanEfficientNetRethinkingModel2019} used blocks discovered using NAS and achieved state-of-the-art performance on the ImageNet dataset while being $8.4\times$ smaller and 6.1$\times$ faster on inference than the previous top solution.
Some other NAS approaches include MnasNet~\cite{tanMnasNetPlatformAwareNeural2019} and EdgeNAS~\cite{luoEdgeNASDiscoveringEfficient2020}, with hardware-aware NAS approaches such as Once-for-All~\cite{caiOnceforAllTrainOne2020} enabling further platform specific DNN architecture tuning.



\subsection{Compression Techniques}

Overall, the best compression technique varied.
Although weight pruning provided a higher compression rates compared to channel pruning, this did not bring speedups in all cases.
We also observed that data-type quantization's speedups were very hardware dependent.

\subsubsection{Pruning}
\label{subsec:discuss:pruning}

For pruning, weight pruning was generally faster than channel pruning; however the former reached achieved a lower proportion of its expected speedups.
There were several cases where a less compressed channel pruning model was faster than a more compressed weight pruning model.
However this appears to come from interactions with a given algorithm, since taking the best variant across algorithms, it was rare for channel pruning to outperform weight pruning.
There were some cases of this on the GPU, and overall the performance of pruned models on the GPUs was worse than on the CPUs.
This makes sense, when we consider the interactions with the hardware.
Namely, sparse computations are irregular, and thus cannot easily take full advantage of the greater number of cores available in a GPU that dense computations can.
Since we could not tuned sparse computations on the GPUs, we cannot comment how well they would perform were the code further optimized.
Other pruning techniques we did not explore include layer-wise pruning, and gradient based methods, the trade-offs of which are discussed in Blalock et al.~\cite{blalockWhatStateNeural2020}.



\subsubsection{Data-type quantization}
\label{subsubsec:discuss_quant}

For our data-type quantization, we observed that the was a negligible impact on accuracy for \texttt{float16}, and a significant drop in accuracy for \texttt{int8}, which was partially recovered using calibration.
We could recover more accuracy using approaches such as quantization-aware training, where we simulate the impact of quantized weights during training, a technique similar to dropout~\cite{srivastavaDropoutSimpleWay2014}.
For \texttt{float16} on the CPUs, we observed a consistent slowdown when compared to \texttt{float32}.
This is because the hardware does not directly support the type, and only runs the computation using software emulation.
Although there are savings in memory footprint, the overhead involved in the emulation clearly outweighs these savings, with the differences exacerbated when tuning.
For \texttt{int8} on the CPUs, we generally observed a speedup, since the CPU ISAs can use SIMD instructions to compute \texttt{int8} computations relatively efficiently.

In the untuned \texttt{int8} case on the CPU, we actually see some cases where we get \textit{higher} than expected speedups, for instance many of the \emph{GEMM} and \emph{direct} cases of the Intel i7 in Figure~\ref{fig:inference_cifar10_cpu}.
The highest of this is for VGG-16 with CIFAR-10 using \emph{GEMM}, where we observe a speedup of over 9.2$\times$.
We hypothesize that using smaller data sizes is reducing cache usage, meaning the algorithm has to fallback to slower caches less in the \texttt{int8} case.
However, this advantage is significantly reduced when we tune.
We believe that Ansor is not fully exploiting the performance potential and search space of \texttt{int8}, since it was
\begin{enumerate*}
    \item initially designed with \texttt{float32} computation in mind, and
    \item \texttt{int8} requires a more complex sequence of instructions to be generated to run efficiently, which Ansor does not appear to factor in.
\end{enumerate*}

For \texttt{float16} on the GPUs, contrasting to the CPUs, we observed in general a reduction in inference time on both GPUs, as they have direct hardware support for \texttt{float16} instructions.
Like the CPU, we also saw speedups with \texttt{int8} models, in general marginally higher than with \texttt{float16}.
However, if we take the best times across all algorithms, we did not see any cases where \texttt{float16} or \texttt{int8} achieved close to an ideal speedup of 2$\times$ and 4$\times$ relative to \texttt{float32}.


In addition to the two quantization types we evaluated, there are other data-types available, such as the emerging DNN-specific \texttt{bfloat16}, or even in the extreme case binarized neural networks~\cite{courbariauxBinaryConnectTrainingDeep2015,hubaraBinarizedNeuralNetworks2016}.
However, in each of these cases, we need appropriate hardware and software support to exploit these types.




\subsection{Algorithms \& Data Formats}

We observed that in the dense case, when tuned on the CPU, \emph{spatial pack} convolution was broadly the best algorithm to use.
When the code was not tuned, the best algorithm varied more.
When tuned on the GPU, in the dense case \emph{direct} convolution was the fastest.
This goes against conventional wisdom, where we would normally expect \emph{GEMM} to be faster on the GPU.
However, we should note that we are using a custom implementation of GEMM within TVM, rather than an optimized BLAS library.
For the pruned algorithms, \emph{GEMM} was typically faster on the CPU, and \emph{direct} was typically faster on the GPU.

One thing to note is that in our evaluation we used the same algorithm for all layers of a given model, in a given evaluation.
However, we could vary the algorithm used per-layer, which could bring significant performance speedups, assuming we can select the best algorithm per layer~\cite{andersonOptimalDNNPrimitive2018}.
We also did not explore all possible convolutional primitives available, such as a class of algorithms that remap the data into the frequency domain using Fourier transformations, such as  Winograd convolution~\cite{lavinFastAlgorithmsConvolutional2016}.
Another dimension that we did not explore was the data-layout.
Commonly, for image data, input data is in either the `channels-first' (\texttt{NCHW}, evaluated in this study), or `channels-last' (\texttt{NHWC}) layout, with a variety of algorithm dependent weight layouts.
Varying the data layout could change the best algorithm significantly.





As discussed in Section~\ref{subsec:discuss:pruning}, for our pruning techniques, we rarely saw the `expected' performance improvements when compared to the dense implementations.
Partly this can be attributed to the inherent overheads of sparse data formats, for example in CSR we need to store up to 3 values for every non-zero element.
This, coupled with irregular data access patterns means that our sparse algorithms may not be exploiting the hardware to the same extent as their dense counterparts,
In terms of data formats, CSR is not the only way to represent our sparsity, and alternative data formats (and their complementary algorithms) may provide different trade-offs.
For example, for channel pruning we could store the weights in a dense format, and store a list of the indices of pruned channels.
Thus our algorithm would run more like our dense computations, with a small overhead for checking if we skip a given channel.
Alternatively, for weight pruning, we could use a format called `block-sparse row' (BSR), which is similar to CSR, however represents blocks of sparse parameters.
In fact, CSR is a special case of BSR where the block-size is one.
This would require having our pruning method to prune blocks of parameters, which would make our weight pruning semi-structured rather than unstructured.
However, this could allow us to reduce the overheads of our sparse storage format, with greater potential savings with larger block sizes, at the risk or higher accuracy degradation.




\subsection{Systems Software}
\label{subsec:discuss:sys_software}


The two main parameters for systems software we considered were compiling with TVM, with and without auto-scheduling.
We generally saw significant speedups when tuning our code, with the best models and compression techniques changing once the code was optimized.
However, we observed no speedup tuning the Xavier.
When testing with server-class NVIDIA GPU platforms available to us, we were observed speedups using auto-scheduling, using the exact same code.
Our conclusion is that some aspect of the AGX Xavier's software stack was incompatible with TVM's auto-scheduling system, but not in a way we could detect.

It is well known that auto-scheduling can provide significant speedups, however the search time required is non-neglible.
We could not collect our auto-scheduled results on the HiKey CPU and GPU for our ImageNet models, since they took too long to tune - over 140 hours each for the two variants we evaluated.
This highlights a key issue with auto-tuning and auto-scheduling systems, namely the cost of search, especially on constrained devices.
Approaches which significantly prune the search space~\cite{tollenaereAutotuningConvolutionsEasier2023} and techniques such as transfer-tuning~\cite{gibsonTransferTuningReusingAutoSchedules2023} can reduce the search time, and potentially increase the speedups.
In addition, auto-scheduling specifically designed for sparse computations could unlock further performance optimizations for our pruned models.

As highlighted in Section~\ref{subsubsec:discuss_quant}, we observed that our pruned models achieved less of a relative speedup once tuned.
A more specialized sparse compiler, such as the emerging SparseTIR system~\cite{yeSparseTIRComposableAbstractions2023} could reduce the impact of these overheads.
This was also observed for our quantized models, which may require similar optimization support.

We experienced an issue compiling 8-bit quantized EfficientNet using TVM, as TVM assumed that in a multiplication operation, only the left-hand operand would be pre-quantized.
However, the structure of EfficientNet violated this assumption, which necessitated a bug-fix which we pushed upstream.
Although a minor issue, it highlights that assumptions systems software can make assumptions about the properties of workloads that may not always hold, especially when novel DNN architectures emerge.

All of our models were defined in PyTorch and evaluated in TVM, however there are other DNN frameworks available, and the relative performance of different DNN frameworks has been well studied~\cite{hadidiCharacterizingDeploymentDeep2019,gibsonOptimizingGroupedConvolutions2020,louloudakisAssessingRobustnessImage2022}.
Other systems-software dimensions to consider are hand-tuned kernel libraries such as OneDNN, cuDNN~\cite{chetlurCuDNNEfficientPrimitives2014}, or other deep learning compiler systems such as TensorRT~\cite{nvidiacorporationNVIDIATensorRTProgrammable2016} or IREE~\cite{theireeauthorsIREE2019}.
Given these choices are an important dimension of DLAS, TVM also allows us to compile using many of these backends, and with its Collage tool~\cite{jeonCollageSeamlessIntegration2023} we can also explore using varying backends for different subgraphs of the same DNN.
In this study, we limited our exploration of this layer, since using TVM's native code generator allowed us to explore other layers of DLAS fairly and systematically.













\subsection{Hardware}
\label{subsec:discuss:hardware}


As expected, the i7 CPU was faster than the HiKey CPU, and the Xavier GPU was faster than the HiKey GPU.
Unfortunately we were unable to see improvements when tuning on the Xavier GPU.
As discussed in previous sections, the hardware is a significant source of variation between solutions, however as we have discussed, it is far from the only one.

Aspects of our hardware that could be better utilized include the big.LITTLE architecture of our HiKey CPU, since we only leveraged the big cores.
Similarly, with the Intel CPU, we did not use hyper-threading, instead ran one thread per core.
With both of these techniques, if used without further across-stack optimizations, it is likely we would see a performance penalty
However, that does not exclude the possibility that better performance could be reached if these features are exploited properly.
For the GPUs, we did not use the Xavier's 64 tensor cores in its GPU, in addition to its 512 general purpose CUDA cores.
In principle, TVM has support for generating code which can exploit these tensor cores, however this requires manual schedule design for each algorithm to exploit the hardware~\footnote{\url{https://tvm.apache.org/docs/how_to/optimize_operators/opt_conv_tensorcore}}.
MetaSchedule~\cite{shaoTensorProgramOptimization2022} allows auto-scheduler search spaces to be modularly expanded to include niche hardware features such as tensor cores, which could allow us to investigate this dimension.

As well as deep learning focused extensions to general purpose hardware such as tensor cores and \texttt{bfloat16} (see Section~\ref{subsubsec:discuss_quant}), are also increasingly seeing deep learning specific hardware accelerators being developed.
These include fixed function accelerators such as the TPU~\cite{jouppiInDatacenterPerformanceAnalysis2017} and others~\cite{harisSECDATFLiteToolkitEfficient2023}; as well as reconfigurable accelerators such as MAERI~\cite{kwonMAERIEnablingFlexible2018} and others~\cite{munoz-martinezSTONNEEnablingCycleLevel2021,stjerngrenBifrostEndtoEndEvaluation2022,chenEyerissV2Flexible2019}.





\subsection{Evaluation Methodology}

For our experiments, we kept our batch size as 1, took the median of 150 runs, disregarding the first warm-up run.
Although this is a common deployment and evaluation scenario, it is important to be aware that this is not the only one, and experimental design should reflect which deployment case is being considered when evaluating models.
For instance, for edge deployment we may expect the batch size to be small, whereas on the cloud it may be large.
Increased batch sizes mean increased memory requirements and inference latency, but also potentially higher throughput.
For our use of 150 runs, disregarding the first run, there could be deployment scenarios where we are more interested in the performance of these initial warm-up runs, before the cache behavior becomes more regular.


==> XX-evaluation_old.tex <==

\section{Evaluation}
\label{sec:evaluation}

For our evaluation, we split our results between CIFAR-10 (Section~\ref{subsec:eval:cifar10}) and ImageNet (Section~\ref{subsec:eval:imagenet}).
We first analyze the accuracy impact of our optimization techniques, then choose maximally compressed models for each technique which maintain accuracy.
We analyze the inference performance of these models using our algorithms and compilation configurations on our CPUs and GPUs.
Section~\ref{sec:discussion} gives a high-level discussion of our results.


\input{fig_neo/fig_tex/acc_cifar10.tex}

\input{fig_neo/fig_tex/model_info_table_cifar10}



\subsection{CIFAR-10}
\label{subsec:eval:cifar10}


\subsubsection{Accuracy}

The models' accuracy with varying levels of compression can be seen in the first row of Figure~\ref{fig:accuracies}.
For the four models, Table~\ref{tab:acc_cifar10} shows the baseline (dense) top-1 accuracy on CIFAR-10.
We observe that for weight pruning (Figure~\ref{fig:acc_unstructured_cifar10}), the accuracy is maintained for all models until 95\% pruning, at which point all models see a drop in accuracy at 99\%.
However, the drop in accuracy for MobileNetV1 and V2 is higher, likely because they have fewer parameters.

We also observe this trend in channel pruning (Figure~\ref{fig:acc_structured_cifar10}), where VGG-16 and ResNet18 maintain their accuracy for longer compared to the MobileNets.
However, for all models the drop in accuracy is earlier compared to weight pruning, with the elbow appearing at 50\% pruning for the MobileNet models, and 80\% for VGG-16 and ResNet18.
We also observe that after the elbow, the drop is higher, to around 10\% accuracy or equivalent to random guessing.

For data-type quantization in Figure~\ref{fig:acc_quant_cifar10}, we observe almost no change in accuracy for \texttt{float16} across our four models.
The output is not bit-wise identical, however at most this represents a 0.03\% difference in top-1 accuracy.
For uncalibrated \texttt{int8} quantization, all models see a drop in accuracy, with MobileNets V1 and V2 seeing the highest drops, to 10.0\% and 16.4\% respectively.
However, with calibration all models recover significantly, with MobileNetV1 losing the most accuracy at 1.7\%.
Table~\ref{tab:acc_cifar10} shows the elbow points of accuracy we take for our inference experiments.



\subsubsection{Inference -- CPU (untuned)}
\label{subsubsec:eval_cpu_inf_untuned}

The first two rows of Figure~\ref{fig:inference_cifar10_cpu} show the untuned performance of our CIFAR-10 models when running on the CPUs of the HiKey (\ref{fig:baseline_hikey_mobilenetv1}-\ref{fig:baseline_hikey_vgg}) and i7 (\ref{fig:baseline_i7_mobilenetv1}-\ref{fig:baseline_i7_vgg}) platforms, with varying compression strategies, and convolutional primitives.
The overall trends, including the fastest combination of parameters under different settings, are shown in Table~\ref{tab:cifar10_results}.
For our untuned baseline, we observe that the i7 and Hikey differ in fastest algorithm, with \emph{direct} and \emph{GEMM} for all models respectively.
However, overall, in most cases across devices, \emph{GEMM} algorithms are the fastest, with one exception for VGG-16 on the Hikey.
In terms of compression techniques, \texttt{int8} has the fastest overall time in three out of four cases on the i7, whereas weight pruning is the fastest on the Hikey in three out of four cases.




If we take the \emph{best} baseline time for each model, we can compute an expected speedup given the compression ratio of each model optimization technique.
For example, on the HiKey for MobileNetV1, with a pruning rate of 95\% we could expect an ideal speedup of 20$\times$.
However, in this case we only achieve a speedup of 2.6$\times$ for our best weight pruning algorithm (\emph{GEMM}), i.e., 13.0\% of our expected speedup.
On average, for weight pruning, we achieve 11.5\% and 21.8\% of the expected speedup on the HiKey and i7 respectively


For channel pruning, the elbow points for our models (see Table~\ref{tab:acc_cifar10}) show that channel pruned models are less compressed than our weight pruning models, which means that we would the latter to always be slower than the former.
However, we observe several cases where a channel pruning model is \emph{faster}, namely for all VGG-16 variants, except for \emph{GEMM} on the HiKey, which is slightly slower.
On average, for channel pruning, we achieve 77.9\% and 83.9\% of the expected speedup on the HiKey and i7 respectively.


For our \texttt{float16} results, we observe a slowdown when compared to the baseline (\texttt{float32}) in every case.
For our \texttt{int8} results, we generally see a speedup relative to the baseline, with some notable exceptions using \emph{spatial pack}.
In some cases, \texttt{int8} gives the best time overall, as seen in the last column of Table~\ref{tab:cifar10_results}.
On average, we achieve 33.6\% and 157.2\% of the expected speedup on the HiKey and i7 respectively.


\input{fig_neo/fig_tex/inf_cifar10_cpu_trans}


\input{fig_neo/tab/cifar10_cpu}


\subsubsection{Inference -- CPU (tuned)}
\label{subsubsec:eval_cpu_inf_ansor}

The last two rows of Figure~\ref{fig:inference_cifar10_cpu} show the tuned performance of our CIFAR-10 models when running on the HiKey (\ref{fig:cpu_tuned_hikey_mobilenetv1}-\ref{fig:cpu_tuned_hikey_vgg}) and i7 (\ref{fig:cpu_tuned_i7_mobilenetv1}-\ref{fig:cpu_tuned_i7_vgg}) CPUs.
Comparing to the untuned results in Section~\ref{subsubsec:eval_cpu_inf_untuned}, we observe that tuning has created some significant differences in the relative performance of our experiments, beyond reducing the inference time significantly.
Focusing on our dense (baseline) models, we observe that \emph{spatial pack} is now the best algorithm in every model on both CPUs, except for VGG-16 on the HiKey where \emph{direct} is slightly faster.

For weight pruning, we observe that sparse \emph{direct} is now the best weight pruning algorithm in every case on both CPUs.
In the untuned case, this is only the case for MobileNets V1 and V2 on the HiKey.
It also outperforms the best dense algorithm (\emph{spatial pack}) in almost every case, with equal performance on the i7 for MobileNetV2.
This is to contrast against the sparse \emph{GEMM} and \emph{spatial pack} algorithms, which are consistently slower than their dense counterparts, reversing the trend for untuned sparse \emph{GEMM}.
On average, we achieve 9.5\% and 6.9\% of the expected speedup on the HiKey and i7 respectively, lower than untuned.


For channel pruning, sparse \emph{direct} is also the best algorithm, and we still observe that in the case of VGG-16, channel pruning is faster than weight pruning in most cases, despite in theory having more operations to compute.
On average, we achieve 39.8\% and 26.6\% of the expected speedup on the HiKey and i7 respectively; again, lower than untuned.

For our \texttt{float16} results, we observe that although there are speedups, we are still slower than the baseline in every case, and these differences are exacerbated when compared to the untuned results.
The speedups of \texttt{int8} on the i7 have disappeared with tuning, with an average slowdown of 2.0$\times$.


\subsubsection{Inference -- GPU (untuned)}

The first two rows of Figure~\ref{fig:inference_cifar10_gpu} show the untuned performance of our CIFAR-10 models when running on the HiKey (\ref{fig:gpu_untuned_hikey_mobilenetv1}-\ref{fig:gpu_untuned_hikey_vgg}) and Xavier (\ref{fig:gpu_untuned_xavier_mobilenetv1}-\ref{fig:gpu_untuned_xavier_vgg}) GPUs.
On the Xavier, dense \emph{direct} convolution is consistently the fastest; whereas on the HiKey it is the best for MobileNetV2 and ResNet18, but \emph{GEMM} and \emph{spatial pack} are faster for MobileNetV1 and VGG-16 respectively.
We also note that the HiKey's inference time on the GPU is much higher than on the CPU.
For example, the baseline \emph{direct} MobileNetV1 is almost 7$\times$ slower when using the GPU.


For our pruned experiments, we see speedups most consistently using \emph{spatial pack}, which is different from on the CPU where we almost always saw a slowdown.
On the HiKey, we see speedups relative to the baseline in multiple cases, and even the fastest possible variant in some cases, such as for channel pruning with \emph{spatial pack} for VGG-16.
In terms of our expected speedup, for the HiKey and Xavier respectively, for weight pruning we achieve 7.4\% and 2.2\%, and for channel pruning we achieve 41.1\% and 26.0\%.



For \texttt{float16}, unlike the CPU, we observe speedups for several cases when compared to our baseline \texttt{float32}.
However, the behavior is not consistent across models, algorithms, or devices.
For example, on the HiKey using \emph{GEMM} with MobileNetV1 (Figure~\ref{fig:gpu_untuned_hikey_mobilenetv1}), \texttt{float16} provides a slowdown, whereas for other models on the HiKey we observe a speedup, as well as a speedup for the same case on the Xavier.
Our most significant slowdown for \texttt{float16} is for ResNet18 (Figure~\ref{fig:gpu_untuned_hikey_resnet18}) using \emph{spatial pack}.
On the Xavier, \texttt{float16} provides a speedup in all cases except for \emph{direct} convolution where we observe small slowdowns.
On average \texttt{float16} achieves 51.9\% and 49.4\% of its potential speedup on the HiKey and Xavier respectively.
The exception to this trend is MobileNetV2 using direct convolution, where we see a small speedup of 1.08$\times$.
For \texttt{int8} quantization, we see a slowdown all instance of direct convolution, speedups for \emph{GEMM}, and speedups for all cases of spatial pack except for MobileNetV1.

\input{fig_neo/fig_tex/inf_cifar10_gpu_trans.tex}
\input{fig_neo/tab/cifar10_gpu}


\subsubsection{Inference -- GPU (tuned)}

The last two rows of Figure~\ref{fig:inference_cifar10_gpu} show the tuned performance of our CIFAR-10 models on GPUs.
As noted in Section~\ref{subsec:setup:sys_software}, we cannot provide tuned results for our sparse models on the GPU.
For \texttt{float32} inference on the HiKey we observe that the inference times for all algorithms are relatively similar, except for VGG-16 where \emph{spatial pack} is significantly slower.
If we take the normalized mean inference time, \emph{direct} is the best for the HiKey.
The HiKey GPU is also still slower than HiKey CPU (tuned), with the best baseline result being 3.1$\times$ slower on average.
For the Xavier, \emph{direct} convolution is the best performing algorithm in all cases.
However, if we compare to the untuned case we see that we do not get any improvement when tuning the Xavier.
We discuss this issue in Section~\ref{subsec:discuss:sys_software}.
For quantization, on the HiKey, taking the best result for each model, we achieve 58.9\% and 44.4\% of the expected speedup on average for \texttt{float16} and \texttt{int8} respectively; the Xavier achieves 49.0\% and 28.4\% of its expected speedups.








\subsection{ImageNet}
\label{subsec:eval:imagenet}


\subsubsection{Accuracy}

For our four models, the baseline (dense) top-1 accuracy on ImageNet is shown in Table~\ref{tab:acc_imagenet}.
EfficientNetB0 has the highest accuracy, which may be surprising given it has fewer parameters.
However, EfficientNetB0 is more recent and thus exploits a number of newer machine learning techniques to improve its parameter and training efficiency.

The accuracy on ImageNet with varying levels of compression can be seen in the second row of Figure~\ref{fig:accuracies}.
We observe a similar trend to our CIFAR-10 models, namely our smaller models (EfficientNetB0 and MobileNetV2) lose their accuracy more quickly than the larger models (DenseNet161 and ResNet50).
We also observe that \emph{all} models lose more accuracy earlier when compared to our CIFAR-10 pruning.
This suggests that our CIFAR-10 models are more overparameterized.

For data-type quantization, we observe a similar trend as CIFAR-10, namely a negligible difference in accuracy for \texttt{float16}.
For ResNet50, we see a large drop in accuracy for uncalibrated \texttt{int8} quantization, recovering to around a 3.0\% accuracy reduction.
For MobileNetV2, we observe a huge drop in accuracy for the uncalibrated model, down to around 0.09\%, recovering to around a 6.6\% accuracy reduction.
This drop was much higher than we expected, so we also tried importing the Keras~\cite{cholletKeras2015} definition of MobileNetV2, and observed the same behavior.

For EfficientNetB0, we also observe a huge drop in accuracy to 0.08\%, however the recovery is much smaller than MobileNetV2's, reaching only 0.43\% accuracy.
This is due to architecture features of the model which make it less suitable for quantization, which we discuss in Section~\ref{subsub:discuss:models}.
For DenseNet161, we cannot run the \texttt{int8} model in TVM due to an unsupported quantized operation.
This excludes it from collection of uncalibrated accuracy and inference time results.
However, when calibrated in ONNXRuntime we reduce accuracy by 1.9\%.


\input{fig_neo/fig_tex/model_info_table_imagenet}


\subsubsection{Inference -- CPU (untuned)}

\input{fig_neo/fig_tex/inf_imagenet_cpu_trans}

The first two rows of Figure~\ref{fig:inference_imagenet_cpu} show the untuned performance of our ImageNet models when running on the i7 and HiKey CPUs.
Focusing on our baseline dense models, we observe that in all cases on the HiKey \emph{GEMM} gives the best performance, which matches its behavior as seen in CIFAR-10 (Section~\ref{subsubsec:eval_cpu_inf_untuned}).
For the i7, \emph{GEMM} is fastest for our large models (ResNet50 and DenseNet161), however \emph{direct} is fastest for our small models (MobileNetV2 and EfficientNetB0); on CIFAR-10 \emph{direct} was consistently the fastest on this CPU.

For weight pruning, we find that by taking our best performing variants as before, we achieve 30.3\% and 41.8\% for the HiKey and i7 respectively; significantly higher than for CIFAR-10.
For channel pruning, this is 60.2\% and 84.2\% respectively, which is 16.7\% less than CIFAR-10 for the HiKey, and 0.3\% more for the i7.
For both weight and channel pruning, we find that the only algorithm which consistently provides a speedup relative to dense is \emph{GEMM}.

For quantization, we see similar trends to CIFAR-10, namely a slowdown using \texttt{float16}, and a speedup using \texttt{int8}.
For \texttt{int8}, we achieve 25.0\% and 73.0\% of the expected speedup on the i7 and HiKey respectively, lower CIFAR-10.

\input{fig_neo/tab/imagenet}

\subsubsection{Inference -- CPU (tuned)}
\label{subsubsec:eval_cpu_inf_imagenet_tuned}

The last row of Figure~\ref{fig:inference_imagenet_cpu} shows the tuned performance of our ImageNet models when running on the i7 CPU.
We note that tuning on the HiKey CPU (and GPU) was not practical, since the two variants we attempted took over 140 hours each, so do not include any of 57 variants required for each device.
For the dense case on the i7, we see that \emph{spatial pack} is the best consistently the best, matching our observed trends on tuned CIFAR-10.
For our pruned models, we do not see any cases where pruned models are faster than a dense \texttt{float32} implementation.
This is contrasted with CIFAR-10, where we observe this in every case.


\subsubsection{Inference -- GPU (untuned)}
\input{fig_neo/fig_tex/inf_imagenet_gpu_trans}

On the Xavier in the dense \texttt{float32} case, we observe that \emph{spatial pack} is the best algorithm for the larger models (ResNet50 and DenseNet161), and \emph{direct} is the best for the smaller models (MobileNetV2 and EfficientNetB0).
On the Hikey, for the smaller models \emph{GEMM} was the best, and for the larger models \emph{direct} was the best.
However, on the HiKey, dense ResNet50 and DenseNet161 experiments using \emph{spatial pack} crashed with the error \texttt{CL\_INVALID\_WORK\_GROUP\_SIZE}.
This means that in one or more layers of these models TVM is exceeding the number of work items our GPU can support (see the OpenCL specification for more details~\cite{stoneOpenCLParallelProgramming2010}).
If we run auto-tuning, TVM can configure the work group size and other GPU parameters, which could avoid this issue.
However, we did not observe this on the Xavier, which has more hardware resources available.

For our sparse experiments, sparse \emph{spatial pack} using weight pruning was consistently the best across both GPUs, however only outperformed the baseline in one case, ResNet50 on the Xavier.
On the Xavier, we found that sparse \emph{direct} experiments did not halt, even allowing hours for a single run.
GPU memory utilization was at its maximum, suggesting that some inefficiency in this algorithm/hardware combination.
Again, auto-tuning may make this variant viable, however as highlighted in Section~\ref{subsec:setup:sys_software}, we cannot tune sparse models on GPUs.

Quantization tends to give speedups compared to dense \texttt{float32}.
Overall, the \texttt{int8} quantized model performs the best on the Xavier, with the \emph{direct} algorithm being the fastest in this case.
On the Hikey, \texttt{float16} \emph{GEMM} is marginally better for EfficientNetB0 and MobileNetV2, and weight pruning \emph{spatial pack} is best for ResNet50 and DenseNet161.


\subsubsection{Inference -- GPU (tuned)}

As discussed in Section~\ref{subsubsec:eval_cpu_inf_imagenet_tuned}, collecting tuned results for the HiKey GPU was not practical.
In addition, we again observed no speedup on the Xavier when tuning, hence we do not include the graphs.

